R2QRec: Learning Recommendation Queries from Retrieval Feedback

Query-based recommendation separates expressing user needs from locating matching items. Its central learning problem is how to turn item interactions into effective retrieval requests when interaction logs do not annotate queries. We present R2QRec, which uses a fixed retrieval system to construct query supervision and evaluate recommendation outcomes. Retrieval verification first selects generated expressions that recover observed items as supervised fine tuning targets, allowing retrieval behavior to determine the target wording. Policy refinement then evaluates generated query sets by the observed item's rank in their fused recommendation list. Log-rank feedback distinguishes outcomes beyond the recommendation cutoff, while a KL penalty constrains policy change relative to the supervised reference. The stages have distinct roles: verification identifies expressions to imitate, and policy refinement improves the combined ranking produced by newly generated queries. Only the query generator is trained; the retriever and item index remain fixed, and no query annotations or learned reward model are required. Across three public datasets, R2QRec achieves state-of-the-art overall recommendation performance among the evaluated methods. Extensive experiments demonstrate the effectiveness of the proposed design and its generalization across generators and domains.

==> figures/R2QRec_Figure1.pdf.name.tex <==
\resizebox{\namedwidth}{!}{%
\begin{tikzpicture}[x=1bp,y=1bp]
\path[use as bounding box] (0,0) rectangle (675.014160,367.511810);
\node[anchor=south west,inner sep=0pt] at (0,0) {\includegraphics{figures/R2QRec_Figure1_namefree.pdf}};
\node[anchor=base west,inner sep=0pt,text={rgb,255:red,18;green,49;blue,62},font={\fontsize{24.6900}{29.6280}\selectfont\sffamily\bfseries}] at (438.916992,8.899994) {(b) \name{}};
\end{tikzpicture}}%


==> figures/fig_closedpool.pdf.name.tex <==
\resizebox{\namedwidth}{!}{%
\begin{tikzpicture}[x=1bp,y=1bp]
\path[use as bounding box] (0,0) rectangle (246.240005,133.199997);
\node[anchor=south west,inner sep=0pt] at (0,0) {\includegraphics{figures/fig_closedpool_namefree.pdf}};
\node[anchor=base west,inner sep=0pt,text={rgb,255:red,32;green,32;blue,32},font={\fontsize{7.5000}{9.0000}\selectfont\rmfamily}] at (180.347519,119.316803) {\name{}};
\end{tikzpicture}}%

